fmiSwap: Run-time Swapping of Models for Co-simulation and Digital Twins

Digital Twins represent a new and disruptive technology, where digital replicas of (cyber)-physical systems operate for long periods of time alongside their (cyber)-physical counterparts, with enabled bi-directional communication between them. However promising, the development of digital twins is a non-trivial problem, since what can initially be adequate models may become obsolete in time due to wear and tear of the physical components, accumulated errors, or the evolving interaction with the environment. As such, there is a clear need for mechanisms that support swapping in new models, as well changing model structures as a whole when necessary. To address this challenge, we propose in this paper a novel artefact, fmiSwap, that is FMI compliant and allows for run-time swapping in standalone co-simulations, where different strategies can be tested easily, as well in fully deployed DT settings with hardware in the loop. We adopt a water-tank case-study consisting of a tank and its controller to demonstrate how fmiSwap works and how it can support swaps in a safe manner.

==> Figures/mabl.tex <==
\lstdefinelanguage{mabl}{
  keywords={typeof, new, true, false, catch, function, return, null, catch, switch, var, if, in, while, do, else, case, break, external},
  keywordstyle=\color{blue}\bfseries,
  ndkeywords={class, export, bool, real, throw, implements, import, this},
  ndkeywordstyle=\color{darkgray}\bfseries,
  identifierstyle=\color{black},
  sensitive=false,
  comment=[l]{//},
  morecomment=[s]{/*}{*/},
  commentstyle=\color{purple}\ttfamily,
  stringstyle=\color{red}\ttfamily,
  morestring=[b]',
  morestring=[b]",
  basicstyle=\scriptsize\ttfamily ,
  numbers=left,
  numberstyle=\tiny,%\ttfamily,
  numbersep=1em,
  xleftmargin=2em,
}
\begin{lstlisting}[language=mabl]
external FMI2Component fmu1, fmu2, fmu3;
external real START_TIME;

bool swapCondition0 = false;
bool stepCondition0 = false;
real jac_current_communication_point_offset0 = 0.0;
while( ((jac_current_communication_point + 
jac_current_step_size) < jac_end_time) )
{
  @Transfer();
  
  swapCondition0 = swapCondition0 || ((fmu2pRealShare[0] 
  - fmu2RealShare[0]) < 1);
  stepCondition0 = stepCondition0 || (true);
  
  fmu1UintVref[0] = 0;
  fmu1RealIo[0] = fmu3RealShare[0];
  fmu1.setReal(fmu1UintVref, 1, fmu1RealIo);
  
  if( (!swapCondition0) )
  {
    fmu2UintVref[0] = 0;
    fmu2RealIo[0] = fmu1RealShare[0];
    fmu2.setReal(fmu2UintVref, 1, fmu2RealIo);
  }
  if( (stepCondition0) )
  {
    fmu2pUintVref[0] = 0;
    fmu2pRealIo[0] = fmu1RealShare[0];
    fmu2p.setReal(fmu2pUintVref, 1, fmu2pRealIo);
  }
  if( (stepCondition0) )
  {
    fmu2p.doStep(jac_current_communication_point_offset0,
    jac_current_step_size, false);
    fmu2pCurrentTime = 
        jac_current_communication_point_offset0 
        + jac_current_step_size;
  }
}
\end{lstlisting}

==> Figures/rbmqspec-1.tex <==
\begin{lstlisting}[language=json]
  "modelSwaps" : {
    "RmqFmu": {
      "swapInstance": "RmqFmu2",
      "stepCondition": "(true)",
      "swapCondition": "(true)",
      "swapConnections": {
        "{RMQ2}.RmqFmu2.speed": [
          "{ACT}.ActuationModel.cmd_speed"
        ],
        "{RMQ2}.RmqFmu2.steering_angle": [
          "{ACT}.ActuationModel.cmd_angle"
        ]
      }
    }
  },
  "modelTransfers" : {
    "ActuationModel": "ActuationModel",
    "KinematicModel" : "KinematicModel",
    "RmqFmu" : "RmqFmu"
  }
\end{lstlisting}

==> Figures/rbmqspec-2.tex <==
\begin{lstlisting}[language=json]
    "stepCondition": "(true)",
    "swapCondition": "(RmqFmu.steering_angle == RmqFmu2.steering_angle)",
\end{lstlisting}

==> Figures/rbmqspec-3.tex <==
\begin{lstlisting}[language=json]
  "stepCondition": "(RmqFmu.steering_angle == RmqFmu2.steering_angle)",
  "swapCondition": "(RmqFmu.steering_angle == RmqFmu2.steering_angle)",
\end{lstlisting}


==> Figures/rbmqspec.tex <==
\begin{lstlisting}[language=json]
{
  "fmus": {
    "{RBMQ}": "./fmus/rbmq_local",
    "{ACT}": "./fmus/unifmu_actuation_model",
    "{KIN}": "./fmus/unifmu_bicycle_kinematic",
    "{RBMQ2}": "./fmus/rbmq_local"
  },
  "connections": {
    "{ACT}.ActuationModel.act_accelleration": [
      "{KIN}.KinematicModel.a"
    ],
    "{ACT}.ActuationModel.act_angle": [
      "{KIN}.KinematicModel.df"
    ],
    "{RBMQ}.RbmqFmu.speed": [
      "{ACT}.ActuationModel.cmd_speed"
    ],
    "{RBMQ}.RbmqFmu.steering_angle": [
      "{ACT}.ActuationModel.cmd_angle"
    ]

  },
  "modelSwaps" : {
    "RbmqFmu": {
      "swapInstance": "RbmqFmu2",
      "stepCondition": "(RbmqFmu.steering_angle == RbmqFmu2.steering_angle)",
      "swapCondition": "(RbmqFmu.steering_angle == RbmqFmu2.steering_angle)",
      "swapConnections": {
        "{RBMQ2}.RbmqFmu2.speed": [
          "{ACT}.ActuationModel.cmd_speed"
        ],
        "{RBMQ2}.RbmqFmu2.steering_angle": [
          "{ACT}.ActuationModel.cmd_angle"
        ]
      }
    }
  },
  "modelTransfers" : {
    "ActuationModel": "ActuationModel",
    "KinematicModel" : "KinematicModel",
    "RbmqFmu" : "RbmqFmu"
  },
  "parameters": {
    "{ACT}.ActuationModel.a1": 0.99889,
    "{ACT}.ActuationModel.a2": -0.0123,
    "{ACT}.ActuationModel.b0": 0,
    "{ACT}.ActuationModel.b1": 0.84766,
    "{ACT}.ActuationModel.b2": -0.834215,
    "{ACT}.ActuationModel.wheel_radius": 0.05,
    "{KIN}.KinematicModel.lf": 0.2,
    "{KIN}.KinematicModel.lr": 0.2
  }
}

\end{lstlisting}

==> Figures/setlinkedvarsalg.tex <==
\begin{scriptsize}
\begin{verbatim}
for each fmu instance
    if instance is source in swap and has existing source ports
        enterif(swapCond.not)
        inst.setLinked() // all ports
    else if instance is target in swap and has swap source ports
        create links from swap source ports to ports
        enterif(stepCond)
        inst.setLinked() // all ports
    else if instance is connected in swap relation
        for each port of instance
        if port is target in swap relation
            if port has existing source port
                enterIf(swapCond.not)
                instance.setLinked(port)
                p.breakLink()
            create link from swap source port to port
            enterIf(swapCond)
            instance.setLinked(p)
        else
            instance.setLinked(p)
    else if instance has source ports
        inst.setLinked()
\end{verbatim}
\end{scriptsize}

==> Figures/swapspec.tex <==
\begin{lstlisting}[language=json]
{
  "fmus": {
    "{x1}": "./fmu1.fmu",
    "{x2}": "./fmu2.fmu",
    "{x3}": "./fmu3.fmu",
    "{x4}": "./fmu2p.fmu"
  },
  "connections": {
    "{x1}.fmu1.o1": [
      "{x2}.fmu2.i2"
    ],
    "{x2}.fmu2.o2": [
      "{x3}.fmu3.i3"
    ],
    "{x3}.fmu3.o3": [
      "{x1}.fmu1.i1"
    ]
  },
  "modelSwaps": {
    "fmu2": {
      "swapInstance": "fmu2p",
      "stepCondition": "(true)",
      "swapCondition": "(fmu2p.o2 - fmu2.o2 <1)",
      "swapConnections": {
        "{x1}.fmu1.o1": [
          "{x4}.fmu2p.i2"
        ],
        "{x4}.fmu2p.o2": [
          "{x3}.fmu3.i3"
        ]
      }
    }
  },
  "modelTransfers": {
    "fmu1": "fmu1",
    "fmu2": "fmu2",
    "fmu3": "fmu3"
  }
}
\end{lstlisting}

==> Figures/wtspec-full.tex <==
\begin{lstlisting}[language=json]
{
  "fmus": {
    "{x1}": "watertankcontroller-c.fmu",
    "{x2}": "singlewatertank-20sim.fmu",
    "{x3}": "leak_detector.fmu",
    "{x4}": "leak_controller.fmu"
  },
  "connections": {
    "{x1}.controller.valve": [
      "{x2}.tank.valvecontrol",
      "{x3}.leak_detector.valve"
    ],
    "{x2}.tank.level": [
      "{x1}.controller.level",
      "{x3}.leak_detector.level"
    ]
  },
  "parameters": {
    "{x1}.controller.maxLevel": 2,
    "{x1}.controller.minLevel": 1
  },
  "algorithm": {
    "type": "fixed-step",
    "size": 0.1
  },
  "modelSwaps": {
    "controller": {
      "swapInstance": "leak_controller",
      "stepCondition": "(true)",
      "swapCondition": "(true)",
      "swapConnections": {
        "{x4}.leak_controller.valve": [
          "{x2}.tank.valvecontrol",
          "{x3}.leak_detector.valve"
        ],
        "{x2}.tank.level": [
          "{x4}.leak_controller.level"
        ],
        "{x3}.leak_detector.leak": [
          "{x4}.leak_controller.leak"
        ]
      }
    }
  },
  "modelTransfers": {
    "controller": "controller",
    "tank": "tank"
  }
}

\end{lstlisting}

==> Sections/drobotti-case.tex <==
\subsection{Desktop Robotti with Time Discrepancy Detection}
In the second experiment, we use the developed model swap mechanism in the development of a DT for a prototype of an agricultural field robot. 
An orchestration synchronisation mechanism (OSA) has been developed~\cite{submitted22} into the Maestro framework that can detect and try to mitigate observed time discrepancies between a PT and a DT. 
The OSA mechanism, has a designated FMU that will detect discrepancies between simulation and wall-clock time based on PT and DT having synchronized wall clocks. 
The introduced detection FMU provides a new out-of-sync output that can be used by other FMUs to get informed of any time discrepancy occurrences and react appropriately. 

\begin{figure}[htb!]
    \centering
    \resizebox{.4\textwidth}{!}{\includegraphics{Figures/RobottiDesktop.jpeg}}
    \caption{The Desktop Robotti.}
    \label{fig:dr}
\end{figure}
In a recent experiment~\cite{submitted22} we use the OSA mechanism in a digital twin development of a desktop version (Desktop Robotti) (Figure~\ref{fig:dr}) of an agricultural field robot (Robotti)~\cite{Foldager&18}, developed by AgroIntelli. The Desktop Robotti enables us to experiment ideas in the lab, at a low cost. 
In the experiment the OSA mechanism enables the DT to temporarily disable sending any data back to the robot in case of an out-of-sync situation, caused by e.g. network degradation. This to prevent the robot to be operating with out-of-sync data from the DT. 


The initial DT of the robot consists of three FMUs. 
A data broker, an actuation model, and a vehicle model. 
The broker FMU enables transmission of data into and out of the co-simulation in real-time. 
It is a wrapper around a RabbitMQ message service client library and was first proposed in \cite{Thule2020a} and later extended in \cite{Frasheri&21}. 
In the experiment, the broker FMU forwards steering controls (steering angle and speed) into the co-simulation matching the controls sent to the robot. 
In addition, it carries safety control commands (like a safety stop command) from the co-simulation back to the robot.

For this experiment, the setup requires the additional OSA FMU for time discrepancy detection and in addition that the broker FMU is updated to handle both an out-of-sync input from the OSA FMU and a \texttt{getMaxStepSize} functionality used for a mitigation part of the OSA mechanism. 
The mitigation uses the \texttt{getMaxStepSize} to attempt larger simulation time steps in order to catch up with the external system.

In the context of model swapping the most interesting part concerns the run-time update of the broker FMU since this is the only component for which a replacement/swap takes place and the swap requires a level of state synchronization with the replaced instance. 
Therefore, in the following we will focus our discussion on the broker FMU replacement. 

	Figure~\ref{fig:rbspec1} shows our initial attempt at specifying the model swap for the broker FMU. 
Only the swap parts are shown, not the entire configuration file. 
Besides the specification of the updated connections, the step and swap conditions are both specified as true - like for the water-tank experiment. 
\begin{figure}[tbh!]
    \centering
    \input{Figures/rbmqspec-1}
    \caption[]{Initial configuration of the RMQFMU model swap.}
    \label{fig:rbspec1}
\end{figure}


Figure~\ref{fig:combo-rbmq1} shows the co-simulation output from the broker FMU restricted to the steering angle data originating from the RabbitMQ server. 
In this experiment, the steering angle is a sine waveform generated by the robot control software. 
The swap specification is provided at simulation time 5sec (magenta line) and since both step and swap conditions are true, the swap is instant.

%\begin{figure}[tbh!]
%    \centering
%    \resizebox{.80\linewidth}{!}{\input{Figures/rbmq1.tex}}
%    \caption[]{Instant swap of RmqFmu for RmqFmu2. Step and swap conditions both true. RmqFmu steering angle output before swap (blue), RmqFmu2 immediately connected output after swap (green).}
%    \label{fig:rbmq1}
%\end{figure}

\begin{figure*}[tbh!]
    \centering
    %\resizebox{.80\linewidth}{!}{\input{Figures/rbmq-combo}}
    \input{Figures/rbmq-combo}
    \caption[]{(a) Instant swap of RmqFmu for RmqFmu2. Step and swap conditions true. RmqFmu angle output before swap (blue), RmqFmu2 immediately connected output after swap (green). (b) Conditional swap of RmqFmu for RmqFmu2. Step condition true and swap conditional. RmqFmu angle output before swap (blue), RmqFmu stays connected output after swap (orange). (c) Conditional swap of RmqFmu for RmqFmu2. Both step and swap conditional. RmqFmu angle output before swap (blue), RmqFmu stays connected output after swap (orange) until swap condition where RmqFmu2 gets connected (green).}
    \label{fig:rbmq-combo}
\end{figure*}

As is clear from the figure, the transition from before the swap (blue) to after (green) breaks continuity in the steering angle output. 
This discontinuity is a result of the instant swap, and indicates that some form of synchronization is required. 
If this swap had been immediately carried out in a real DT setting it might have caused unforeseen problems since the DT would be missing a portion of real operational data. 
A stand alone co-simulation, including the upgraded broker FMU from the start, would also not have been showing this issue.
However, being able to simulate the real swap in a co-simulation setting, 
provides means
% allows 
to investigate and mitigate such issues up front. 
% Also, a stand alone co-simulation including the upgraded broker FMU from the start would not have been showing this issue.

To remedy the issue, the swap condition is changed such that the output steering angle of the existing broker FMU must match the output of the replacement FMU. 
The resulting co-simulation output is given in Figure~\ref{fig:combo-rbmq2}, and the corresponding (updated) swap specification part is shown in Figure~\ref{fig:rbspec2}.
%The updated swap specification part is shown in Figure~\ref{fig:rbspec2} and the resulting co-simulation output in Figure~\ref{fig:combo-rbmq2}.

%\begin{enumerate}
%\item NTP has synced. Enabling the OSA feature means also going from a state where NTP is not necessarily started to one where it is. And to have safe outputs of the OSA FMU we cannot enable it until NTP state is in sync.
%\item The RabbitMQ FMU queues in the two instances must be consistent. When enabling the new RabbitMQ FMU, its queue will be initially empty, whereas the original RabbitMQ FMU may have messages already in its queue. Hence the original RabbitMQ FMU may be able to step (given some proper maxage) whereas the new FMU cannot step yet. And until both produce same outputs, the swap can’t happen.
%\end{enumerate}

\begin{figure}[tbh!]
    \centering
    \input{Figures/rbmqspec-2}
    \caption[]{Second configuration of the RmqFmu model swap.}
    \label{fig:rbspec2}
\end{figure}

%\begin{figure}[tbh!]
%    \centering
%    \resizebox{.80\linewidth}{!}{\input{Figures/rbmq2.tex}}
%    \caption[]{Conditional swap of RmqFmu for RmqFmu2. Step condition true and swap conditional. RmqFmu steering angle output before swap (blue), RmqFmu stays connected output after swap (orange).}
%    \label{fig:rbmq2}
%\end{figure}
In the output it can be seen that after the swap (timestep 5s), the RmqFmu and RmqFmu2 outputs are both following the sine wave, but the outputs are offset by a constant 5s time interval. 
Thus, the original RmqFmu keeps being connected and is not replaced by RmqFmu2. 

The real issue is caused by the RmqFmu having an internal queue state. 
When enabling the new RmqFmu2, its queue will be initially synchronized to contain the next unacknowledged message from the server. 
The original RmqFmu may have messages already in its internal queue that are read and acked with the server and thus the new RmqFmu2 instance may read and output an initial message from the server being later than all (not yet processed) messages in the RmqFmu incoming queue. 

To remedy this issue, we can make use of the step condition of our specification language, by stating that the RmqFmu2 steering angle must be synchronized with the RmqFmu output before stepping. 
I.e.\ RmqFmu2 will initialize and synchronize its first message with the RabbitMQ server. Thereafter, it
will start stepping only when the original RmqFmu has processed any messages in its queue. 
Finally, we allow RmqFmu2 to be swapped in at this instant, so the step and swap conditions are set equal. 
The resulting output and corresponding specification can be seen in Figure~\ref{fig:combo-rbmq3} and Figure~\ref{fig:rbspec3}, respectively.

In the simulation output it can be seen, that at simulation time 5s when the swap specification is enabled, the output used until time 10s is from the original RmqFmu FMU (orange).
The step condition of RmqFmu2 is enabled at time 10s and the swap condition also becomes enabled so the output used is from RmqFmu2 (green). Using the step and swap conditions in this manner provides a replacement behaviour of the RmqFmu that correctly preserves the input signal. Our model swapping mechanism allowed us to experiment safely with alternative models in a co-simulation setting prior to any real deployment.

\begin{figure}[tbh!]
    \centering
    \input{Figures/rbmqspec-3}
    \caption[]{Final configuration of the RmqFmu model swap.}
    \label{fig:rbspec3}
\end{figure}

%\begin{figure}[tbh!]
%    \centering
%    \resizebox{.80\linewidth}{!}{\input{Figures/rbmq3.tex}}
%    \caption[]{Conditional swap of RmqFmu for RmqFmu2. Both step and swap conditional. RmqFmu steering angle output before swap (blue), RmqFmu stays connected output after swap (orange) until swap condition where RmqFmu2 gets connected (green).}
%    \label{fig:rbmq3}
%\end{figure}


%\gita{As we discussed it makes sense to run the actual experiment with the desktop robotti and record a video that will go along with the submission. Also I think Lukas mentioned this, we can upload the recorded data somewhere, such that a reviewer/reader can replicate the experiments :). I am just putting this comment here so that we don't forget :).}

==> Sections/reflections.tex <==
\section{Reflections on Applicability}
%To support a safe update, the updated controller can be modelled and run-time swapped into the existing co-simulation to test the effect even before updating the real DT. 
%Our model swap mechanism allows us to (i) test in co-simulation the effect of run-time swapping the control strategy and also (ii) play with different strategies. 
%Thereby providing confidence in the upgraded models prior to deployment in a real uninterruptible DT setting. 

==> Sections/relwork.tex <==
\section{Related Work}\label{sec:relwork}

Developing Cyber-physical systems is a cumbersome task involving modelling physical interactions of software systems as well as the interaction among different networked, embedded systems. One of the key approaches to reduce the development complexity for CPS is Model-driven Engineering (MDE)~\cite{mohamed2021model}. With MDE, systems are developed using compositions of models. This allows for rapid adaptations of developed systems by replacing individual models, leading to a blurry boundary between development and deployment~\cite{baresi2010disappearing}. A specific challenge comes about swapping models in Cyber-physical systems (CPS) where the computational system has to directly interact, verify, and control physical properties whether they are of discrete or continuous nature~\cite{esterle2016cyber}.

J{\o}rgensen~\cite{JORGENSEN1986} proposed structural dynamic models, the creation of larger models by combining simple, small-scale models. In addition, allowing adjustments of their parameters through control mechanisms. 
%This idea has been improved with considering the discontinuities in differential equations~\cite{oren1987model}, taxonomies for multi-models~\cite{Barros1997}, or multi-models specifically for multi-agent systems~\cite{yilmaz2004dynamic}.
% This was extended by discontinuities~\cite{oren1987model}, taxonomies~\cite{Barros1997}, and static multi-models~\cite{yilmaz2004dynamic}. 
Several extentions have been proposed over the years: \"Oren~\cite{oren1987model} considered the discontinuities in the differential equations of models and how to model them, while Barros~\cite{Barros1997} proposed taxonomies to model multi-models. Yilmaz and \"Oren~\cite{yilmaz2004dynamic} introduce multi-models specifically for multi-agent systems. 
%
%%%Ref below GOES away
%Uhrmacher~\cite{Uhrmacher2001} introduces an implementation-independent formalism for models whose description entails the possibility of changing their own state and behaviour utilising transition functions as part of the models. However, the approach is not directly applicable to CPSs and the continues domain.

Nilsson and Giorgidze~\cite{nilsson2010exploiting} proposed functional hybrid modelling as an approach to non-causal modelling to switch between pre-defined models.
%%%Ref below GOES away
%At around the same time, Zimmer~\cite{zimmer2010equation} developed equation-based language to explicitly define adaptations in variable-structure systems, i.e., models where equations change during the time of execution.
%Mehlhase \cite{Mehlhase2014} proposes to utilise models with multiple, different modes. She further introduced a Python-based framework allowing to switch between different modes of the model. The framework utilises end values from the previous mode to initialise the new mode when switching between them.
%In contrast, we allow to dynamically change the model structure and introduce new models and underlying model structures at runtime without suspending the simulation.

% {\color{red}Many have proposed multi-models and structurally dynamic models~\cite{nilsson2010exploiting}.}

% \cite{mustafee2018hybrid} proposes hybrid systems modelling as extension to hybrid simulations, where techniques such as Agent-based simulations, System Dynamics, Discrete Even Simulation, and Monte Carlo Simulations are combined.

Replacing or swapping models in MDE, after systems have been deployed, is not entirely new. 
The work on models{@}run.time~\cite{blair2009models} has introduced the idea of replacing individual models while the actual system is executed. This allows for runtime adaptation of the behaviour of the respective system. The need for explicit mechanisms and approaches to implement this runtime change is highlighted by Bennaceur et al.~\cite{bennaceur2014mechanisms} or G\"otz et al.~\cite{gotz2015adaptive}, among others.
The recent and very extensive survey on models{\@}run.time~\cite{bencomo2019models} highlights the challenge of replacing models during runtime.
%
%%%Ref below GOES away
%Fouquet et al.~\cite{fouquet2012dynamic} propose an approach to replace models at runtime in CPS but focus on memory utilisation and reboot delay when adding new firmware. They do not explicitly consider the dynamics and continuous change to which an CPS is exposed.%, which is tackled with our proposed approach.

Heinzemann et al.~\cite{heinzemann2019transactional} present 
% an extension to their existing
a modeling language which allows to specify platform-independent models of hierarchical re-configurations. Their reconfiguration protocol guarantees atomicity, consistency, and isolation properties and real-time constraints by design. Furthermore, it can be utilised to verify properties in discrete and continuous physical environments.

%%%Ref below GOES away
%When developing self-adaptive systems which will undergo changes after their deployment, the underlying adaptation needs to be defined and implemented as well. Goldsby et al.~\cite{goldsby2008goal} propose different levels of requirements engineering and respective processes including a dedicated level for adaptation scenarios and adaptation infrastructure engineering. 

%%%Ref below GOES away
%Trusting autonomous adaptive systems able to change their own behaviour is often challenged due to the limited predictability of the systems~\cite{andras2018trusting}. Zhang and Cheng~\cite{zhang2006model} introduces formal models for adaptive systems enabling verification of the systems state before and after the adaptation. They focus on verification of software behaviour resulting from collaborative of multiple software components. In a similar way, Han et al.~\cite{han2020easymodel} proposed a refinement-based modelling and verification approach for self-adaptive systems.

Bellman et al.~\cite{bellman2021self} highlight the importance of self-integrating systems and their ability to master continuous change. They argue that models need to be able to replace models during execution. With changing models and underlying software, we also have to reconsider our testing approaches in a dynamically changing world. Bertolino and Inverardi~\cite{bertolino2019changing} highlight the challenges and outline approaches to tackle them. We argue that not only models need to be replaced but also model structures need to be adaptable at runtime and tested accordingly.

% Recently, Gomes et al.~\cite{modelica.org:Gomes:2021a} present the FMI 3.0 standard and specifically disuss the different types of clock-based simulations. They discuss synchronous clocked simulations and scheduled execution, where the former utilises a common clock for all events while the latter relies on real-time simulation of black-box models.

%%%Ref below GOES away
%Finally, Brockhoff et al.~\cite{brockhoff2021process} discuss the potential of process mining for process discovery and even process prediction. While this is not directly related to adapting simulation models and replacing models at runtime, the outlined approaches could be utilised to automatically identify changes in processes and trigger a model exchange dynamically.









% References: \cite{Mehlhase2014, Barros2003, Barros1997, Uhrmacher2001, modelica.org:Gomes:2021a}

% models\@runtime \cite{blair2009models, gotz2015adaptive, bencomo2019models}

% highlighting the need for adaptation mechanisms \cite{bennaceur2014mechanisms, gotz2015adaptive} without a solution


%\henrik{The concept of \textit{variable-structure models (VSM)} has been studied in the context of simulation in e.g. \cite{Mehlhase2014}. This appears related although not within FMI and also more isolated to changing mode of a single model during co-sim. The VSM needs pre-defined and pre-processed by tool. In contrast we consider dynamic change of co-sim structure (not pre-defined) with runtime validation and transitions.} 

%\henrik{References (from Claudio): \cite{Mehlhase2014, Barros2003, Barros1997, Uhrmacher2001, modelica.org:Gomes:2021a}}



==> Sections/rmqfmu.tex <==
\subsection{RMQFMU: A bridge to the real world}
There are cases in which it is desirable to feed data -- live or historical -- to a co-simulation.
As an example, consider the case in which a user would like to build a DT using the aforementioned co-simulation tools.
In this scenario, the co-simulation/DT should be able to connect to the external world, \eg to a piece of hardware or a fully-developed robot, and exchange data back and forth in real-time. 
To enable such bi-directional communication, we have proposed in previous work the RMQFMU~\cite{rmqfmu21}, an AMQP based FMU that serves as a data-broker between a co-simulation and any external system able to send/receive data through a RabbitMQ server.

RMQFMU can be configured through a set of parameters, covering the connection to the server, such as username and password, as well as other parameters that shape its internal behaviour, such as the \textit{maxage} among others, which refers to the age of the data to be considered valid in the DT.
Additionally, it is possible to specify the inputs and outputs of the FMU through its model description file. 
The RMQFMU steps in time when it has valid data from an external source, and sets its outputs to the received values. 
Conversely the FMU will send data to an external listener every time its inputs are set to a value different to those in the previous time-step. 
